Fairness Through Domain Awareness: Mitigating Popularity Bias For Music Discovery

As online music platforms grow, music recommender systems play a vital role in helping users navigate and discover content within their vast musical databases. At odds with this larger goal, is the presence of popularity bias, which causes algorithmic systems to favor mainstream content over, potentially more relevant, but niche items. In this work we explore the intrinsic relationship between music discovery and popularity bias. To mitigate this issue we propose a domain-aware, individual fairness-based approach which addresses popularity bias in graph neural network (GNNs) based recommender systems. Our approach uses individual fairness to reflect a ground truth listening experience, i.e., if two songs sound similar, this similarity should be reflected in their representations. In doing so, we facilitate meaningful music discovery that is robust to popularity bias and grounded in the music domain. We apply our BOOST methodology to two discovery based tasks, performing recommendations at both the playlist level and user level. Then, we ground our evaluation in the cold start setting, showing that our approach outperforms existing fairness benchmarks in both performance and recommendation of lesser-known content. Finally, our analysis explains why our proposed methodology is a novel and promising approach to mitigating popularity bias and improving the discovery of new and niche content in music recommender systems.

==> Sections/03aDataset.tex <==
\section{Dataset Augmentation Procedure} \label{sec:data_aug}

% \genre{this is actually something you should highlight in the paper -- i think this subsection deserves an entire section (put it before methodology). it is a new dataset and you should talk about (1) why existing datasets are not good, (2) how you construct these datasets and their uniqueness, (3) how you plan to manage them (release it publicly?)}
% \rebecca{Fill in motivation - there are few standardized, feature compatible datasets. Also, literally every version of LastFM is different - different people use different filtering techniques and so it's super hard to check.}

An important limitation of working on music recommendation is the scarcity of up-to-date, publicly available \textit{feature-based} datasets. Though numerous datasets are available, a majority remain purely interaction-based. Thus, in order to facilitate a \textit{domain-aware} approach,  we extensively augment two prominently used, publicly available datasets: LastFM (LFM) \cite{LFM} and Million Playlist Dataset (MPD) \cite{MPD}. We select these two datasets in particular for their breadth and relevance towards a broad range of settings related to music recommendation. First, they encompass two important levels of recommendation: playlist- (MPD) and user- (LFM) based. The decreased granularity of user-level interactions (LFM) is significantly less homogeneous, and therefore innately noisier, than that of a unified playlist (MPD). Second, they showcase two different methods of user feedback data: implicit and explicit. MPD consists of user generated playlists. Thus, positive MPD interactions indicate genuine content affinity as signalled by the a user's explicit selection of a particular in the construction of a playlist. Meanwhile, LFM contains interactions consist of all content that a user engaged with and the positive nature of these interactions is \textit{inferred implicitly}. Crucially, implicit interactions have no guarantee of relevance, making the dataset more prone to noise. 

Since both datasets consist of exclusively interaction data, we augment both of our datasets to include a rich set of features scraped from Spotify API~\cite{spotipy}. To achieve this, we draw on a large body of work from the music information retrieval community (MIR) \cite{foote_content_1997, geleijsne_quest_2007}. The details of the augmented features are as follows:
\begin{enumerate}
% \vspace{-\baselineskip}
    \item \textbf{Sonic features.} Spotify has a series of 9 proprietary features which are used to define the audio elements associated with a track. They are \textit{danceability, energy, loudness, speechiness, acousticness, instrumentalness, liveness, valence, and tempo}. Each of these features is a continuous scalar value. In order to normalize the scales, we apply $10$ leveled binning to the values where bin $0$ marks the lower end of the spectrum and bin $9$ is the highest. 
    \item \textbf{Genre features.} The notion of genre has long been used to categorize musical content. In our case, we identify the primary artist associated with each song and use their unique identifier to collect all the tags associated with them. In each of the datasets, there are approximately 5K unique tags. We select the top $20$ and convert them to a one-hot encoding.
    \item \textbf{Track Name features.} For each song in the dataset, we extract the song title and pass it through a pre-trained language transformer model, \emph{BERT} \cite{devlin2019bert}, into an embedding of dimension $512$.
    \item \textbf{Image features.} For each song in the dataset we extract the associated album and, using the unique identifier, download the image associated with it. Finally, we pass this image through a pre-trained convolutional neural network, \emph{ResNet50} \cite{resnet50}, to generate an embedding of dimension $1024$.
\end{enumerate}
We will publicly release the constructed datasets, the construction code, along with the code for using various feature sets, in our repository upon the publication of this paper.

==> Sections/Old_Versions/00abstract.tex <==
As online music platforms grow, music recommender systems play a vital role in helping users navigate their vast musical databases. However, many of these systems have a major design flaw called popularity bias through which recommender systems favor mainstream content over, potentially more relevant, but niche items \jian{a bit too negative by saying `design flaw', how about something like: However, these systems suffer from popularity bias through which recommender systems favor mainstream content over, potentially more relevant, but niche items?}. Such disparities in item visibility can cause issues both from a performance perspective and a societal one. In this work, we propose a domain-aware, individual fairness-based approach which addresses popularity bias in graph neural network (GNNs) based recommender systems. We fine-tune item representations learned by a GNN recommender \jian{let's use the term consistently, GNN recommender vs. GNN based recommender system} using music features and define an individual fairness regularizer \jian{can we say `define xxx regularizer'? it's proposed in REDRESS paper. can we say `and impose individual fairness to reflect ...'?} to reflect a ground truth listening experience, i.e., if two songs sound similar, this similarity should be reflected in their representations. We apply our methodology \jian{let's think about a name for your method.} to two discovery \jian{the term `discovery' has never appeared before so people may wonder what discovery based tasks mean. can we rewrite the second sentence (the `However, ...' one) to briefly mention discovery? something like they cannot *discover* more niche items because of popularity bias.} based tasks, performing recommendations at both the playlist level and user level. Then, we ground our evaluation in the cold start setting, showing that our approach outperforms existing fairness benchmarks in both performance and recommendation of lesser-known content. Finally, our analysis explains why our proposed methodology is a novel and promising approach to mitigating popularity bias and improving the discovery of new and niche content in music recommender systems.

==> Sections/Old_Versions/01introduction.tex <==

As our content consumption habits shift towards online spaces, the sheer quantity of content on streaming platforms has created an \textit{attention economy} \cite{Lanham_economics_2006} in which the economic standing of an online content provider is measured by its ability to garner attention from online users \cite{yang_visualization_2003, korth_database_1997}. Within the music domain, this movement has cemented algorithmic curation as one of the major value propositions that music streaming platforms can offer their user base \cite{drott_why_2018, Mok_Way_Maystre_Anderson_2022}. In this way, recommender systems have been cast into the role of gatekeepers, guiding the relationships formed between users and artists \cite{prey_locating_2020, odair_beyond_2020}. Due to the significant role that these systems play in the discovery and interactions with musical content, the architectural decisions made within these systems have massive ripple effects on the way content is created and consumed \cite{born_artificial_2021}. 

In recent years, the analysis of various recommender systems has shown the presence of a particularly worrisome disparity: that of popularity bias \cite{jannach_what_2015, park_long_2008, steck_item_2011, chen_bias_2020}. This bias occurs when algorithmic reliance on pre-existing data causes new, or less well known items, to be disregarded in favor of previously highly rated items. % items which were previously highly rated. 
Such prioritization can have multifaceted effects on the various stakeholders in the recommender system domain. From the user perspective, popularity bias has been shown to manifest itself in poor service towards users with niche tastes \cite{ekstrand_cool_2018, nicola}. Meanwhile, from the producer or musicians' perspective, popularity bias can create harmful feedback loops that disenfranchise artists from minority classes or those serving minoritarian tastes \cite{ferraro_break_2021}. Finally, from the societal perspective, popularity bias can have dramatic consequences on the kinds of art that is produced since the attention metrics which are used to train recommender systems are also often used as metrics for the payment of artists \cite{bauer_music_2017, born_artificial_2021}. And so, our work takes on the task of \textbf{mitigating popularity bias} in music recommendation. 

% \begin{wrapfigure}{R}{0.6\textwidth}
%   \begin{center}
%     % \includegraphics[width=.4\linewidth]{Viz/Example2.png}
%     \includegraphics[width=.4\linewidth]{Viz/graph.png}
%   \end{center}
%    \caption{\textbf{Illustrative Example of Popularity Bias}: For each song track, $t_i \in T_{OG}$, we generate a counterfactual song, $t_i^{*} \in T_{CF}$, by duplicating the feature set of $t_i$ and adding it to the graph via a single randomly selected edge. In Section \ref{sec:emb},  we apply 2-dimensional PCA and analyze the distance between the learned embeddings of the original, $T_{OG}$, and counterfactual, $T_{CF}$, sets. We show that approaches without mitigation will show a larger distance between the learned representations of the groups $T_{OG}$ and $T_{CF}$, thus showing the presence of popularity bias in a learned representation}\label{fig:ill_ex_total}
%   \label{fig:ill_ex1}
% \end{wrapfigure}

% \begin{wrapfigure}{r}{0.6\textwidth}
    
%     \centering
    
    
   
%     % \includegraphics[width=.5\linewidth]{Viz/CF_ill.png}
%      % \includegraphics[width=.5\linewidth]{Viz/REDRESS-4.png}
%     % \subcaption{\textbf{Popularity Bias in Recommendation}}
%     % \label{fig:ill_ex2} 
   

%

% \begin{wrapfigure}{r}{0.6\textwidth}
%     % \begin{minipage}{\linewidth}
%     \centering\captionsetup[subfigure]{justification=centering}
%     \includegraphics[width=.4\linewidth]{Viz/Example2.png}
%     \subcaption{\textbf{Node Centrality as Popularity Bias}}
%     \label{fig:ill_ex1}
%     % \includegraphics[width=.5\linewidth]{Viz/CF_ill.png}
%      % \includegraphics[width=.5\linewidth]{Viz/REDRESS-4.png}
%     % \subcaption{\textbf{Popularity Bias in Recommendation}}
%     % \label{fig:ill_ex2} 
   
% % \end{minipage}
% \caption{\textbf{Illustrative Example of Popularity Bias}: For each song track, $t_i$, we generate a counterfactual song, $t_i^{*}$, by duplicating the feature set of $t_i$ and adding it to the graph via a single randomly selected edge.  We apply 2-dimensional PCA and analyze the distance between the learned embeddings of the original, $T_{OG}$, and counterfactual, $T_{CF}$, sets. As we will show later in Section \ref{sec:emb}, approaches without mitigation will show a larger distance between the learned representations of the groups $T_{OG}$ and $T_{CF}$, thus showing the presence of popularity bias in a learned representation}\label{fig:ill_ex_total}
% \end{wrapfigure}

Our work focuses on the role that popularity bias can play in the process of discovering novel and relevant music. A significant body of work has shown that users whose listening habits are governed by algorithmic curation expect an algorithm to help them discover music that is relevant to their taste \textit{which they would not have found for themselves} through a manual search \cite{villermet_follow_2021, drott_why_2018, Mok_Way_Maystre_Anderson_2022, cunningham_more_2006}. Thus, in order to empower this form of algorithmic musical exploration, a recommender system must be both robust to mainstream, majoritarian listening patterns and have a nuanced awareness of the musical tastes among individual listeners. And, from this perspective, mitigating popularity bias goes hand in hand with the latent performance objective of facilitating discovery because a skew towards popular content can complicate the suggestion of unfamiliar musical options. We apply our mitigation technique to graph neural network (GNN) based recommender systems due to their ability to smoothly interpolate between macro (communal) and micro (individual) consumption patterns while also integrating item level information \cite{wu_graph_2020}. In the graph space, popularity of individual items is deeply interlaced with a node's centrality, or the number of outgoing edges that leave this node and connect it to others in the graph. This is because the innate process of representation learning is affected by the number of neighbors a node has \cite{kang_rawls_2022}. And, thus, a node's centrality can dictate the quality of its learned representation. This suggests that duplicating the feature information of an extremely popular song, creating a new song using these duplicate features, and randomly placing it once at the edge of a graph, will significantly impact its likelihood of recommendation, even if everything about the song remains \textit{exactly the same}. This can be incredibly problematic because if the goal of discovery is to find content that fits a user's musical taste, then the task of providing fresh recommendations is rooted in the ability of an algorithm to build rich and expressive representations for all items, irrespective of their centrality in a consumption graph. Thus, in this setting, we argue that the gold standard is an algorithm that can successfully identify a user's favorite popular music before it became mainstream. To illustrate this motivation, we present the following simulation. Consider the most popular song track by a listener's favorite artist. Then, consider how a popularity focused recommendation system would have treated this song before it became mainstream. Had their consumption been governed solely by such an algorithm - would they have discovered this song or even this artist? Furthermore, recognizing this kind of feature-based similarity among a collection of songs requires an approach that is grounded in the musical domain. Thus, we define a domain aware, individual fairness based approach that uses music features to fine-tune item representations such that they reflect information that is, in essence, a ground truth to the listening experience: if two songs sound similar, this similarity should be, at least somewhat, reflected in their representations.

We compare our individual fairness-based method with three other methods which are grounded in other canonical fairness notions, group and counterfactual fairness \cite{barocas-hardt-narayanan}. As we show in our results, by promoting individual fairness among songs, we are able to improve the likelihood of diverse, relevant, and niche content recommendation. To do this, we harness the power of a graph based individual fairness framework, REDRESS \cite{dong_individual_2021}, extend it to a bipartite setting, and integrate it into the end to end training pipeline of a GNN based recommender system called PinSage \cite{ying_graph_2018}. We take two publicly available datasets and extensively augment them to generate a set of nuanced multi-modal track features. Using these novel feature sets, we ground our perspective of individual fairness in the notion of musical similarity and show the effects of our method at balancing between content- and context-based music representation. Finally, through a series of empirical results, we show that our fairness framework enables us to outperform a series of accepted fairness benchmarks in both performance and recommendation of lesser known content on two important music recommendation tasks. 

In summary, the contributions of this work are threefold. First, we present a novel perspective on the environment in which popularity bias should be evaluated by grounding our problem formulation in the cold start, discovery setting. In doing so, we propose a nuanced definition of popularity and show how its application can provide deeper insight into performance/fairness tradeoffs in music datasets. Second, we propose a domain aware, individual fairness based method for mitigating popularity bias and show its effectiveness on two real-world music recommendation tasks. Third, in order to facilitate domain awareness, we take two classical, interaction-based music datasets and augment them to provide reproducible multi-modal graph data. Together, these contributions show how valuable domain awareness can be for mitigating popularity bias and motivate the need for future work in this direction.


==> Sections/Old_Versions/02related_work.tex <==
\section{Related Work}
\jian{(1) it is better to have some connecting words here; (2) overall this section is too long -- right now it is 1+ pages, we should try to make it within 1 page, ideally 0.75 page;}
\subsection{Defining Popularity Bias} \label{sec:pop_def_rw}
\begin{figure}
  \begin{center}
    \includegraphics[width=0.3\textwidth]{Viz/LT.png}
  \end{center}
  \caption{Classic Long Tail Definition\cite{abdollahpouri_controlling_2017}}
  \label{classic_LT}
\end{figure}

\jian{let's only have 2 subsections: popularity bias in recommender systems (merge the first two sections, shorten the length) and GNNs in recommendation}
Most broadly, popularity bias refers to a disparity between the treatment of popular and unpopular items at the hands of a recommender system. As such, this term is loosely tied to a collection of complementary terms including exposure bias \cite{Diaz__evaluating_2020}, superstar economics \cite{bauer_music_2017}, long tail recommendation \cite{mansoury_graph_2021}, the Matthew effect \cite{moller_not_2018}, and aggregate diversity \cite{adomavicius_improving_2012, celma_novel_2008}. An important preliminary step to the analysis and mitigation of this bias is a quantitative definition for popularity. In general, the notion of popularity is intrinsically linked to the visibility of items or the exposure that an item may receive in a ranked list. One body of work defines popularity with respect to individual items' visibility. For example as a probability of an item appearing in the training data \cite{Zhang_causal_2021} or the likelihood of interaction with an item given its position in a list \cite{Diaz__evaluating_2020, mansoury_graph_2021}. However, one of the difficulties of this approach is the extreme ranges that these values can have making it difficult to normalize for adequate comparisons \cite{gruson_offline_2019}. Another group of approaches attempts to simplify this process by applying some form of binning to the raw appearance values. Most notably, the long tail model \cite{celma_from_2008, goel_anatomy_2010, downey_evidence_2001, yang_visualization_2003, park_long_2008} has risen to prominence as a popularity definition. \jian{this is a bit weird, how about moving it to introduction or methodology, where we want to talk about existing works' limitations. in related work, we should focus on talking about difference to existing works, but not their limitations.}As shown in Figure \ref{classic_LT}, we can see that the first 20\% of items, called \textit{short head}, take up a vast majority of the user interactions and the remaining 80\%, or \textit{long tail} and \textit{distant tail}, have, even in aggregate, significantly fewer interactions. Often, splitting items into the \textit{short head} and \textit{long tail} (either including or removing \textit{distant tail}) to define disparity in popularity can overcome the issues of range while still representing concrete disparities in item level visibility. Intuitively we can see that these two approaches define two ends on the spectrum of granularity. In this work, we propose a novel definition of popularity (see Section \ref{sec:pop_def}) that is positioned in the intersection between these two methodologies. We show that our method is able to bridge the gap between raw appearance values and binary notions of popularity and motivate its design by the nuanced insights it allows in explaining fairness/evaluation trade offs.



\subsection{Mitigating Popularity Bias} 
There has been a lot of work done analyzing and codifying the nature of popularity bias in recommender systems \cite{canmares_should_2018, Jadidinejad2019HowSI, jannach_what_2015, chen_bias_2020}. Approaches to mitigating popularity bias are often grounded in one of three methods: \textbf{pre-processing}, where modifications are made to debias input data \cite{boratto_interplay_2021}, \textbf{in-processing}, where modifications to the loss function are made to debias the parameters \cite{rhee_countering_2022, wei_model_2021, zheng_2021_disentangling}, or \textbf{post-processing}, where the output of a recommender model is re-ordered to mitigate position bias \cite{abdollahpouri_managing_2019, mansoury_graph_2021}. Mitigation strategies can also be characterized by their underlying fairness notions. For example, using \textbf{group fairness} \cite{barocas-hardt-narayanan} preprocessing techniques sample from the minority population to balance their representation in the training interactions \cite{boratto_interplay_2021, schnabel2016recommendations}. Or, various in-processing methods modify loss functions to regularize for group imbalances \cite{rhee_countering_2022, zhang_incorporating_2023}. Finally, various post-processing methods use re-ranking \cite{abdollahpouri_managing_2019, Zehlike_fair_2017}. Alternatively, many approaches use \textbf{counterfactual fairness} to disentangle the effect of popularity on a recommender system's score \cite{wei_model_2021, zheng_2021_disentangling, Zhang_causal_2021}. In comparison with group and counterfactual fairness, there has been relatively little work done in relation to \textbf{individual fairness}. This is due to the difficulty of defining a similarity through which to define pairs of individuals. In their work, \citeauthor{Chakraborty2017FairSF} define similarity on the basis of relevance, proposing a method in which items are given exposure that is proportional to their predicted relevance. In a more recent work, \citeauthor{wang_providing_2022} define similarity between learned representations, however, their work is grounded in knowledge graph based recommendation and thus cannot be applied to many recommendation settings.

\jian{this part is way too long. majority in the related work section should be related work.}There are a few key elements that distinguish our method from this body of work. Firstly, none of these methods approach fairness from a domain-aware angle. Rather, the definitions of fairness are grounded in an abstract space that can be applied in a domain agnostic way to various settings (as shown by the choices of datasets in each of these works). Of course, there are many domains in which item and user level features are scarce, sparse, or non existent and these require fairness definitions to be unaware of individual attributes. However, in an environment like music streaming where there is a plethora of valuable feature information, we believe that grounding fairness notions in domain specific attributes can prove incredibly valuable. Second, we distinguish our approach to individual fairness from that applied in the previous works. As mentioned in our introduction, our approach to mitigating fairness is grounded in the notion of discovery that algorithmic curation can provide. If we consider the gold standard to be an algorithm that can successfully identify an example of a user's favorite, popular song before it became mainstream, then even an individual fairness method that uses the output of a recommender model, whether it be in learned representation \cite{wang_providing_2022} or the relevance score \cite{Chakraborty2017FairSF}, is already influenced by an item's popularity. Similarly, a group fairness approach \cite{rhee_countering_2022, abdollahpouri_managing_2019}, which focuses on equity between popularity groups would actually intensify this divide because, in becoming mainstream, an artist's work could switch groups (and thus be treated very differently). Finally, the approaches that consider counterfactual perspectives are perhaps the most likely to perform well in our setting, however, we will show that in the cold start setting, where there is little known about a user's preference, it can be difficult to estimate an individual's propensity towards popular or unpopular items. 


\subsection{GNNs in Recommendation} \label{sec:GNN_in_rec}
In recent years various graph neural network (GNN) architectures have been proposed for the recommendation domain \cite{wu_graph_2020}. For brevity, we will focus only on the two methods that are used as the backbone recommenders to the fairness mitigation techniques discussed later in this paper. In particular, \emph{PinSage} \cite{ying_graph_2018} is an industry solution to graph-based recommendation. Unlike many competing methods, which train on the entire neighborhood set of a node, PinSage trains on a randomly sampled subset of the graph. In order to construct neighborhoods, PinSage uses $k$ random walks to select the top $m$ most relevant neighbors to use as the neighbor set. However, it is important to note that PinSage learns representations of items but not users. Thus, this architecture was followed by many methods in which user and item embedding are both learned in the training process. \emph{LightGCN} \cite{he_lightgcn_2020}, is one such method and, since its proposal in 2020, it is still considered state of the art. The ability of this method to learn both item and user representations simultaneously allows it to excel on metrics such as recall or NDCG where the exact user/item interactions must be recovered in order to achieve high performance. Crucially, unlike PinSage which integrates item level features into its training regime, LightGCN is neither domain aware nor inductive, meaning that it is not necessarily state of the art in settings, like the music domain, where new users and items are added on a daily basis. As we will discuss, in Section \ref{sec:discussion}, the choice of underlying recommender model can deeply shape both the fairness definitions and the fairness mitigation that can be achieved during recommendation. 

==> Sections/Old_Versions/03methodology.tex <==
\section{Methodology}

\subsection{Recommendation Scenario} \label{sec:prob_def}
As user consumption habits have shifted away from albums and towards playlists, streaming companies have invested significant energy into the task of \textit{Automatic Playlist Continuation} and \textit{Weekly Discovery} \cite{schedl_current_2018, stanisljevic_impact_2020}. In the first task, \textit{Automatic Playlist Continuation} requires the recommender system to perform \textit{next $k$ recommendation} on a user generated playlist. Meanwhile, in \textit{Weekly Discovery}, rather than augmenting a specific playlist, an algorithm is tasked with the creation of a new  playlist based on a user's aggregated listening habits. We will now formally define both settings. 

\begin{definition}
    Automatic Playlist Continuation: Given a set of playlists, $P = P_{train} \bigcup P_{valid} \bigcup P_{test}$ and a set of songs (or tracks) $T$, for each playlist in the test set, $p_i \in P_{test}$, we have a set of songs,  $\{ t_j : t_k \in p_i \}$, we can divide this set into $t_{peek} \bigcup t_{holdout}$ using the positions of the songs in the playlist. Thus, our goal is, to predict the held out song tracks, $t_{holdout}$, given only the first $t_{peek}$ songs for each playlist, $p_i \in P_{test}$. 
\end{definition}

\begin{definition}
    Weekly Discovery: Given a set of users, $U = U_{train} \bigcup U_{valid} \bigcup U_{test}$ and a set of tracks $T$, for each user in the test set, $u_i \in U_{test}$, we have a set of songs,  $\{ t_j : t_k \in u_i \}$, we can divide this set into $t_{peek} \bigcup t_{holdout}$ using the timestamps at which a user interacted with a song. Thus, our goal is, to predict the held out song tracks, $t_{holdout}$, given only the first $t_{peek}$ songs for each user, $u_i \in U_{test}$. 
\end{definition}
Having defined these two settings, for brevity, we will be using playlists and users interchangeably in future definitions since they are treated similarly in our two datasets. It is important to note that our setting is also grounded in the cold start scenario as defined by \citeauthor{schedl_current_2018}. This means that the training, validation, and test splits are performed by random sampling without replacement from the user (or playlist) pool. Thus, during the evaluation phase, the only information available about a test user (or playlist) are the songs in $t_{peek}$. In this way, we are able to integrate the temporal nature of music consumption and move our evaluation closer to the online setting in which it would be interacting with users. Furthermore, we simulate the real world situation in which new users are joining the platform and require relevant, unbiased recommendations without providing a large body of their previous interaction data. It is exactly at this junction, before a user's musical preference solidifies, that the need to mitigate popularity bias is most acute because once a majoritarian pattern has been installed in a user's embedding, it will continue to influence all further recommendations. 

\subsection{Popularity Definition}\label{sec:pop_def}
\begin{figure}
  \begin{center}
   \includegraphics[width=.3\textwidth]{Viz/Binning_LFM_logscale.png}
   \includegraphics[width=.3\textwidth]{Viz/Binning_MPD_logscale.png}
  \end{center}
 \caption{\textbf{Binning Procedure for Popularity Definition}: we show the breakdown of the bin locations for both dataset. In doing so, we motivate the need for the application of logarithmic smoothing by showing the popularity patterns which become visible once such a transformation is applied. Furthermore, we show the increased granularity that an increased number of bins applies. \jian{try to see if we can put 2 figures in one row; if so, make the font size of axis labels and legends bigger}}
\label{fig:bin_breakdown}
\end{figure}
We will now explain our unique formulation of popularity and then motivate it with respect to previous works and the needs of our setting. We use the following steps to define our popularity setting. First, we count the number of times each song track, $t_i$ appears within the playlist (or user) training interactions such that for each $t_i$, $a_{t_i} = |\{p_i : t_i \in p_i \}|$. Then, we apply the base $10$ logarithmic smoothing to these values such that for each $t_i$, $pop_{t_i} = log_{10}(a_{t_i})$. Finally, we apply binning onto these values to split them into 10 groups such that for each $t_i$,  $pop\_bin(t_i) \in \{0, 1, ..., 9\}$ where bin $9$ has a higher popularity value than bin $0$. The visualization of this binning procedure and its comparison with the long tail method can be seen in Figure \ref{fig:bin_breakdown}. As demonstrated by our visualizations, transforming the raw values into the logarithmic space shows that the bins are filled in relatively even intervals. Similar to the classic long tail model, as the popularity increases, so does the number of songs included in a bin.
In relation to methods described in Section \ref{sec:pop_def_rw}, we combine the best of each methodology. Using raw values provides information about each individual song. Using a logarithmic transformation to the raw values provides a solution to the scaling issues while allowing for granular comparisons. Meanwhile, binning allows us to provide aggregate statistics that highlight large scale patterns in the recommendations. Our motivation behind selecting $10$ bins is twofold: First of all, as we will show in Section \ref{sec:b_arch} our extension to the REDRESS framework involves synthetically inflating pairwise similarity values by the distance of their popularity bins. Since we find that rescaling our similarity values to be between (1, 10) increases the performance of the REDRESS framework, using bins with the same range allows for simple integration into our framework. Furthermore, since the canonical popularity bias definition rests on the binary long tail model, our methodology allows us to maintain a similar power law distribution while still providing more granular insight into the degrees of user preference at different levels of popularity. As we show in the visualizations provided in Figure \ref{fig:dset_breakdown}, applying our binning methodology to our two datasets showcases crucial differences in the preference distribution of the two training sets. As we will explain in our results section, these differences become an important standpoint through which to interpret results. For example, in the MPD dataset, we can see that there is already an intrinsic preference shown towards items in the lowest popularity bin. This means that the fairness/performance tradeoff will be lower than that of LFM where there is a clear priority given to mid-level popularity songs. 

% \golnoosh{For consistency, please change the title of the plots in Figure 3 to be bold and match figure 4}
% \golnoosh{the title, and the axis of these plots are not readable.}
\begin{figure}[h]
\centering
\includegraphics[width=.24\textwidth]{Viz/log10_upref_LFM.png}
\includegraphics[width=.24\textwidth]{Viz/LT8020_upref_LFM.png}
\includegraphics[width=.24\textwidth]{Viz/log10_upref_MPD.png}
\includegraphics[width=.24\textwidth]{Viz/LT8020_upref_MPD.png}
\caption{\textbf{Dataset Breakdown by Long Tail Definition}: We show visualizations of the user preferences indicated in the training set for each of the datasets used in evaluation. Using the classic Long Tail model, where there are only two bins (short head/long tail) can mask nuanced differences between datasets which can influence the underlying consumption patterns. However, adding more bins and applying logarithmic scale helps to visualize differences in the datasets, which, in turn, helps explain fairness/performance tradeoffs. \jian{two possible ways to display these figure: (1) 2 rows, 2 figures per row; (2) 4 figures in one row (use figure* environment)}}
\label{fig:dset_breakdown}
\end{figure}



\subsection{Dataset Augmentation} \label{sec:data_aug}
Beginning with both tabular datasets, we follow the following two steps: (1) create a  bipartite graph structure, and (2) define complex node level features. In the case of LastFM (LFM)  \cite{LFM}, we use users and songs to define the two node types which are connected by edges when a user has interacted with a song. In the case of the Million Playlist Dataset (MPD) \cite{MPD}, the nodes represent playlists and songs with an edge indicating that a song is contained within a playlist.  It is important to note that both datasets consist of exclusively interaction data, in the form of user, and item pairs. Thus, in order to facilitate a domain aware graph based recommender system, we augment both of our datasets to include a rich set of features scraped from Spotify API \cite{spotipy}. To achieve this we draw on a large body of work from the music information retrieval community (MIR). For example, it is common to use acoustic features to categorize musical items based on their frequencies \cite{foote_content_1997} or genres \cite{geleijsne_quest_2007}. In addition to these two perspectives, we also add song titles and album artworks to capture references to cultural phenomena or associations that can influence a listening experience. Unfortunately, due to space constraints, we were unable to include our ablation studies regarding the use of various feature sets but the code for them will be included in our code repository. \\ 
\indent \textbf{Sonic features} 
Spotify has a series of 9 proprietary features which are used to define the audio elements associated with a track. They are danceability, energy, loudness, speechiness, acousticness, instrumentalness, liveness, valence, and tempo. Each of these features is a continuous scalar value. In order to normalize the scales, we apply $10$ leveled binning to the values where bin $0$ marks the lower end of the spectrum and bin $9$ is the highest. \\
\indent \textbf{ Genre features }
The notion of genre has long been used to categorize musical content. In our case, Spotify offers artist level genre tags. Thus, for each song, we identify the primary artist associated with this song and use their unique identifier to collect all the tags associated with them. In each of the datasets, there are approximately 5K unique tags. We select the top $20$ and convert them to a one-hot encoding.\\ 
\indent \textbf{ Track Name features } 
For each song in the dataset, we extract the song title and pass it through a pre-trained language transformer model, \emph{BERT} \cite{devlin2019bert}, into an embedding of dimension $512$. \\ 
\indent \textbf{ Image features } 
For each song in the dataset we extract the associated album and, using the unique identifier, download the image associated with it. Finally, we pass this image through a pre-trained convolutional neural network, \emph{ResNet50} \cite{resnet50}, to generate an embedding of dimension $1024$.


\subsection{Recommender Architecture}\label{sec:ps_arch}
The task of performing recommendation in the graph space can be seen as extending the task of link prediction to a bi-partite graph. Here, link prediction is done on an undirected graph $G = (V,E)$. For brevity, we will be using playlists and users interchangeably since they are treated similarly in our two datasets. Thus, in both cases, $V = T \bigcup P$ is a set containing song (or track) nodes, $T$, and playlist (or user) nodes, $P$ (or $U$). Edges $E$ are defined between a playlist $p_k$ (or user $u_k$) and a song $t_i$ if $t_i$ is contained in $p_k$ (or listened to by $u_k$). The task of link prediction in this setting involves using 2-hop neighborhoods to predict whether song nodes $t_i, t_j \in T$ share a common parent playlist $p$. In our implementation, we make a few deviations from the originally proposed architecture. Unlike \citeauthor{ying_graph_2018} who use curriculum training to increase the difficulty of negative samples with each increasing epoch, we use uniform random sampling. In order to compensate for this potential loss of information, we use focal loss \cite{lin_2018_focal}, rather than margin loss, to train the network. The premise of focal loss is that, due to the construction of the function, it penalizes mistakes on harder examples. We experiment with both losses and find that focal loss significantly improves the performance of the model. It is important to note that since the potential benefits or drawbacks of PinSage as a general recommender system are out of the scope of this paper, we do not focus on the performance gains that such a change might provide. 



\subsection{REDRESS} \label{sec:r_arch}


\emph{REDRESS} is an individual fairness framework proposed by \citeauthor{dong_individual_2021} for learning fair representations in single node graphs. In our work, we extend this framework to the bipartite recommendation setting and integrate it into our popularity bias mitigation approach. We will begin by giving some intuition into the framework and then provide the mathematical details of its formulation. The general mindset of individual fairness is that items which are similar in the input space should remain similar in the output space \cite{dwork2011fairness}. 

% \begin{figure}{R}{0.4\textwidth}
%   \begin{center}
%     \includegraphics[width=0.4\textwidth]{Viz/REDRESS-2.png}
%   \end{center}
%   \caption{\textbf{Visualization of the REDRESS framework}: here we look at the similarities between a central node, $t_i$, and two neighboring nodes, $t_u, t_v$. We show the initial similarity matrix, $S_G$, and the learned similarity matrix, $S_Z$. Using these similarities we generate each matrix to rank all the items $t_k$ with respect to their similarity with the central node, $t_u$. As we can see in this example, since the ordering of $t_i$ than $t_v$ in the respective lists has changed, individual fairness (as defined in our work) does not hold.}
%   \label{fig:REDRESS}
% \end{figure}

% \golnoosh{I don't think this visualization is an added value, let's remove it. }

In the graph setting, individual fairness can be interpreted to mean that nodes which were similar in their initial feature space should remain similar in their learned representation embeddings. In order to use individual fairness to fine-tune node level embeddings, we require a formulation of similarity that is both relevant to our setting and differentiable. Broadly, principles of individual fairness suggest that similarity should be based on domain expertise. In their implementation \citeauthor{dong_individual_2021} use cosine similarity between features to define as a proxy for expert domain knowledge. However, in our work, we use only the music features as the basis for cosine similarity comparisons. In this way, our similarity notion is domain aware and grounded in the essence of musical experiences: acoustics. Thus, when applied to the music setting, song nodes containing acoustically similar music features are expected to remain similar once they have been passed through the representation learning paradigm of PinSage. In order to cast pairwise cosine similarity as a differentiable function, \citeauthor{dong_individual_2021} take a probabilistic approach inspired by the methodology used in learning to rank \cite{burges_lambda_2010}. Formally, we can express individual fairness, as it is used in this work, in the following definition:


\begin{definition}(REDRESS: Individual fairness). Given some similarity metric $s(., .)$, an apriori pairwise similarity matrix, $S_G \in \Re^{|T| \times |T|}$, and a learned pairwise similarity matrix, $S_{Z} \in \Re^{|T| \times |T|}$, defined by applying $s(.,.)$ to the learned graph representations, $\hat{Y}$, we say the predictions are individually fair if for each instance $i$, the ranked list generated from $S_{Z}$ is consistent with the ranked list generated from $S_G$. 
\end{definition}

More concretely, for each song node, $t_i$, and node pair $t_u, t_v$ in a graph $G$, we can define their similarities, based on the cosine similarity metric $s(., .)$ in which we input their music features from the input feature collection, $X[v] \in \Re^9$ or learned embedding, $Z[v] \in \Re^{m}$. Applying this procedure in a pairwise fashion, we can derive two matrices. The first is termed the \textit{apriori similarity}, $S_G$, in which similarity is calculated using vectors of input music features that are independent of the GNN model, $M$. The second is termed the \textit{learned similarity}, $S_{Z}$, in which similarity is calculated between learned embeddings generated by the training process of a GNN model, $M$. In essence, for every song node $t_i$, we can define its similarity with two neighboring song nodes $t_u, t_v$ as $S_G[i,u]$ and $S_G[i, v]$ in the case of $S_G$ or $S_Z[i, u]$ and $S_Z[i, v]$ in the case of $S_{Z}$. In order to make comparisons between these matrices differentiable, we define two probability tensors that encode the each similarity pair, $S_G[i,u], S_G[i,v]$ as a probability that node $t_i$ is more similar to node $t_u$ than $t_v$. That is, using the values in $S_G$ and $S_{Z}$ we define two probability matrices, $P_G \in \Re^{|T| \times |T| \times |T|}$ and $P_Z \in \Re^{|T| \times |T| \times |T|}$.  Thus, for each individual node, $t_i$ and two other nodes selected from the remaining graph, $t_u, t_v$, the \textit{apriori} probability, $P_G$, which is based on exclusively musical similarities, $S_G$, is defined as: 
\vspace{-1mm}
\begin{align*}
    P_G[u,v, i]= \begin{cases}
  1  & S_G[i,u] > S_G[i,v] \\
  0 & S_G[i,u] <= S_G[i,v]
    \end{cases}
\end{align*}
\vspace{1mm}
And the \textit{learned} probability, $P_Z$, which is based on similarities in the learned embedding space, $S_Z$, is defined as: 
\begin{align*} 
    P_Z[u,v,i] = \frac{1}{1 + \exp\Bigl({-\alpha(S_Z[i,u]-S_Z[i,v]}\Bigr)}
\end{align*}
where $\alpha$ is a scalar which can be treated as a hyperparameter. Having defined the two tensors using a probabilistic approach, we can now train for fairness by using standard cross entropy loss. Thus, for each node $t_i$, we define: 
\begin{align*}
    L_{t_u,t_v}(t_i) &= -P_G[u,v,i] \log P_Z[u,v,i] - (1 - P_G[u,v,i]) \log (1 -  P_Z[u,v,i]) 
\end{align*}
And over all the nodes $t_i \in V$: 
\begin{align*}
    L_{fairness} = \sum_{i}^{|T|} \sum_{u}^{|T|}\sum_{v}^{|T|} L_{t_u,t_v}(t_i)
\end{align*}
In their work, \citeauthor{burges_lambda_2010} found that adding a weighting factor based on the changes in NDCG to restrict modifications to changes in the top $k$ values of each ranked list can improve performance and decrease the computational complexity of this calculation. Thus, redefining the loss above to only focus on the top-k, we define: 
\begin{align*}
    L_{fairness} = \sum_{i}^{|T|} \sum_{t_u\in |topk(i)| } \sum_{t_v \in |topk(i)|}L_{t_u,t_v}(t_i) |\triangle NDCG_{@k}|_{u,v}
\end{align*}
where $\triangle$ represents the change in NDCG between the two lists. Finally, the broad process of training occurs using two stages: utility based loss and utility and fairness based loss as follows: 
\begin{align*}
    L_{total} = L_{utility} + \gamma L_{fairness}
\end{align*}
where $\gamma$ is a scalable hyperparameter which controls the focus given to fairness and can be used to select a balance between utility and fairness during the second training phase. 




\subsection{BOOST} \label{sec:b_arch}
As it is formulated, the REDRESS framework does not explicitly encode any attributes of popularity in its training regimen. Thus increases in visibility given to niche items comes only from innate similarities in the musical features, not explicit promotion of niche content. To extend this technique to explicitly counteract popularity bias, we define the \textit{BOOST} technique which is used to further increase the penalty on misrepresentation of items that come from diverse popularity categories. More formally, given the learned representation matrix, $S_Z \in \Re^{|T| \times |T|}$, we define another matrix $B$ in which 
\begin{align*}
B_{ij} = |pop\_bin(i) - pop\_bin(j)|
\end{align*}

Thus, in the \textit{BOOST} loss formulation, in place of $S_Z$ we use $S_Z' = S_Z + B$. 
% Thus, the representations will only be heavily penalized if the apriori similarities in $S_G$ are very far apart from the synthetically increased values of $S_Z'$. 

\subsection{Generating Recommendations} \label{sec:rec_gen}
Given that PinSage learns representations on the item level, we need to define a procedure for generating user (or playlist) embeddings. As mentioned in Section \ref{sec:prob_def} where we defined the recommendation scenario, for each test user (or playlist), $u_i$ we have a set of tracks $\{t_i : t_i \in u_i\} = t_{peek} \bigcup t_{holdout}$. Thus, in order to generate a user (or playlist) embedding we define: $z_{u_i} = MEAN( \{ z_{t_j}: t_j \in t_{peek} \}) $ where the $z_{k} \in \Re^{1 \times d}$ are the learned representations of dimension $d$. We then apply cosine similarity with all the available tracks and select the top-k items by their score. 

==> Sections/Old_Versions/04experiments.tex <==

\section{Experiments}
\subsection{Datasets}
We evaluate our approach on two music datasets, LastFM (LFM) \cite{LFM} and the Million Playlist Dataset (MPD) \cite{MPD}. Table \ref{table:dataset_stats} presents the graph statistics of each datasets. We are limited by the number of publicly available music datasets which are compatible with our feature augmentation procedure. However, in selecting these datasets we cover a broad range of settings in which music recommendation can be evaluated. First, we define two important levels of recommendation: playlist (MPD) and user (LFM) based. Furthermore, we select two methods of feedback data: implicit and explicit. MPD consists of user generated playlists meaning that interactions consist of songs which are explicitly pronounced as relevant due to the explicit nature of a user selecting the song for their playlist. Meanwhile, LFM contains user/song interactions that are gathered by aggregating all the songs that a user clicked on (even if they did not necessarily finish or enjoy the content). Thus, these implicit interactions have no guarantee of relevance,  making the dataset more prone to noise. And, particularly in the cold start setup, this can significantly increase the difficulty of making predictions because implicit interactions are less indicative of a user's latent taste and less homogeneous in nature than that of a unified playlist. 


\begin{table}[h] %PS vs LFM TABLE
\centering
\footnotesize
\begin{tabular}{|l|c|c|c|c|c|}
\hline 
Dataset &Recommendation Setting & Feedback Type & \#Users/Playlists & \#Songs & \#Artists \\
\hline 
\hline
MPD & \textit{Automatic Playlist Continuation} &Explicit& 11,100& 183,408 & 37,509\\ 
\hline 
LFM & \textit{Weekly Discovery} &Implicit & 10,267 & 890,568 & 100,638 \\ 
\hline 
\end{tabular}
\caption{Breakdown of Dataset Statisctics}
\label{table:dataset_stats}
\vspace{-8mm}
\end{table}

\subsection{Evaluation}
In addition to the classic recommendation metrics such as Recall and NDCG, which focus on rewarding a system for correctly guessing the exact track that is located in a test playlist, we design a series of metrics to assess the performance from a musical perspective and popularity bias mitigation. Table \ref{table:metrics} presents the details of the formulation of these metrics. Next, we provide the motivation behind each metric. Thus, for a ground truth set, $G$, and a recommended set, $R$, we define the set of unique artists in a playlist as $arid(.)$ and the $d$-dimensional musical feature matrix associated with the tracks of a playlist as $mus(.) \in \Re^{|.| \times d}$. 

\begin{table}[h]
\renewcommand{\arraystretch}{2.5}
\centering
\footnotesize
\begin{tabular}{|c|c|c |}
\hline 
\textbf{Metric} & \textbf{Category} & \textbf{Formulation} \\
\hline 
\hline
\textbf{Artist Precision@100} & Music&$Artist\_Recall = \frac{1}{|P|}\sum_{p \in P_{test}}\frac{|arid(G_p) \cap arid(R_p)|}{|arid(G_p)|}$ \\ 
\hline 
\textbf{Sound Homogeneity@100} &Music& $Flow = \frac{1}{|P|}\sum_{p \in P_{test}} cosine\_sim(mus(Z_{t_i}), mus(Z_{t_i})) ~  \forall (t_i, t_j) \in R_p$ \\ 

\hline 
\hline 
\textbf{Artist Diversity (per playlist)} & Fairness & $Diversity =  \frac{1} {|P|} \sum_{p \in P_{test}} \frac{|\{arid(R_p)\}|}{|arid(P)|}$ \\ 
\hline
\textbf{Percentage of Long Tail Items} & Fairness&$\%LT =  \frac{1}{|P|} \sum_{p \in P_{test}} \frac{|\{t_i: t_i \in R_p \cap t_i \in LT\}|}{|p|}$ \\ 
\hline
\textbf{Coverage over Long Tail Items} &Fairness & $LT\_CVG =  \frac{|\{t_i: t_i \in R_{P_{test}} \bigcap t_i \in |LT| |} {|LT|}$\\ 
\hline
\textbf{Coverage over Artists} & Fairness& $Artist\_CVG =  \frac{|\{arid(t_i): t_i \in R_{P_{test}}|} {|ARID|}$\\ 
\hline 
\end{tabular}
\caption{Breakdown of Music and Fairness Performance Metrics}
\label{table:metrics}
\vspace{-10mm}
\end{table}

% \golnoosh{can you make a table for all the metrics? You can make one with two columns, where the first column is the name of the metric and the second one is the equation}
\subsubsection{Music Performance Metrics}
The purpose of these metrics is to broaden the scope of evaluation to include hidden positive hits. The motivation for using \emph{Artist Precision} is that we believe identifying the correct artist is a parallel task in music recommendation \cite{korzeniowski_artist_2021}. The second metric, \emph{Sound Homogeneity}, is meant to indicate the musical cohesiveness of the recommended songs in a playlist \cite{bontempelli_flow_2022}.  

\subsubsection{Fairness Metrics}
To assess the performance of our recommendations on the promotion of long tail songs and artists, we draw on a series of metrics which have been previously used to evaluate the fairness performance of a model \cite{abdollahpouri_managing_2019, Patro_fairrec_2020, celma_from_2008}. Percentage based metrics capture the ratio of niche to popular content that is being recommended on a playlist (or user) level. Meanwhile, \emph{coverage} looks at the aggregate sets of niche songs and artists over all recommendations. For example, if a recommender has a high percentage but low coverage, this means that the same niche items are being selected many times. Meanwhile, if an item has high coverage but a low percentage, it means that the algorithm is selecting a diverse set of niche content but recommending it very rarely. Thus, the gold standard is a high percentage and high coverage in both niche songs and artists.  


\subsection{Baselines}
We select five baselines to compare our performance: \\ 
First, we use two naive baselines:  \textbf{(1) Features}: Instead of the learned representations, we use the raw feature vectors in the recommendation methodology presented in Section \ref{sec:rec_gen} and \textbf{(2) MostPop}: For each dataset we select the $100$ most popular tracks and recommend them for each of the test playlists (or users). Then, we select three state of the art fairness mitigation techniques:  \textbf{(1) ZeroSum}\cite{rhee_countering_2022}: In their work \citeauthor{rhee_countering_2022} use group fairness to modify the BPR, pairwise similarity, loss \cite{he_lightgcn_2020} by including a regularization term which forces scores within negative and positive item groups to remain close. Following their original implementation, we select LGCN as it is the state of the art in graph based recommender systems.  \textbf{ (2) MACR}\cite{wei_model_2021}: In their work \citeauthor{wei_model_2021} use counterfactual estimation to denoise for the effects of popularity bias in user and item embeddings. They propose a three branch structure in which, in addition to learning user and item embeddings, they also learn a constant that indicates the causal effects of an item's score on a user and item embedding. Here too, we follow their methodology and use LGCN \cite{he_lightgcn_2020} as the underlying recommender system, and \textbf{(3) Smooth xQuAD}\cite{abdollahpouri_managing_2019}: In their work \citeauthor{abdollahpouri_managing_2019} propose a post-processing method which aims to re-rank the items in a recommended list to account for improved diversity. They propose an extension to the original xQuAD \cite{santos_exploiting_2010} framework which uses a re-ranking appraoch to greedily select items to balance the diversity ratio the re-ranked list. 
\subsection{Experimental Setup}
Each of the baseline methods was tested with learning rates  $\sim (0.01, 0.0001)$, embedding sizes of $[10, 24, 64, 128]$ and batch sizes of $[256, 512, 1024]$. The best LGCN performance was achieved using a batch size of $512$, a learning rate of $0.0001$, and an embedding layer of size $10$ (for MPD) and $24$ (for LFM). For the values in the tables below, each stochastic method was run $5$ times and averaged. All details and further hyperparameter settings can be found on our GitHub repository \footnote{preliminary version:~ \url{https://anonymous.4open.science/r/RecSys23-9B7F/README.md}}.  

==> Sections/Old_Versions/05results.tex <==
\section{Results}
The purpose of our evaluation is to analyze whether domain aware individual fairness can contribute to the mitigation of popularity bias. 
% We consider the downstream effects on artist representation and how they are affected by the integration of song-level individual fairness. Finally, we compare our method with all the five baselines presented above and provide a holistic analysis of its performance among various performance and fairness metrics. 
In doing so, we answer the following research questions:
\begin{itemize}[noitemsep,topsep=0pt]
    \item [RQ1]: How does incorporating individual fairness improve the mitigation of popularity bias?
    \item [RQ2]: Do the effects of individual fairness propagate to the producer (artist) level? 
    \item [RQ3]: How does our individual fairness approach compare to existing methods for mitigating popularity bias? 
\end{itemize}
\subsection{RQ1: How does incorporating individual fairness improve the mitigation of popularity bias?}\label{sec:emb}
To showcase the performance of our algorithm in the discovery setting and motivate the need for individual fairness in the mitigation of popularity bias, we present an illustrative example and then simulate it on the MPD dataset. We evaluate how much popularity bias contributes to differences in learned representations of popular and unpopular duplicates of individual items.

\begin{figure}[h]
\vspace{-4mm}
\centering
\includegraphics[width=.25\textwidth]{Viz/EMB/PS_CF.png}
\includegraphics[width=.25\textwidth]{Viz/EMB/SR_CF.png}
\includegraphics[width=.25\textwidth]{Viz/EMB/MACR_CF.png}
\includegraphics[width=.25\textwidth]{Viz/EMB/R_CF.png}
\includegraphics[width=.25\textwidth]{Viz/EMB/B_CF.png}
\caption{\textbf{Simulating Popularity Bias}:  We select $100$ of the most popular songs in the Million Playlist Dataset, duplicate their node level features, add them with new song track ids, and connect them using a randomly selected edge to one playlist. We apply 2-dimensional PCA to the item embeddings learned by each recommendation method. Then, we analyze the distances between the embedding group centroids. We find that REDRESS and BOOST have the lowest distance between the original, popular and duplicated, unpopular track groups, showing the least amount of popularity bias.}
\label{fig:cf_emb}
\vspace{-4mm}
\end{figure}

For each song track, $t_i \in T_{OG}$, we generate a counterfactual song, $t_i^{*} \in T_{CF}$, where everything about the features is \textit{exactly the same} and the only difference is that $t_i$ appears in many playlists while $t_i^{*}$ appears only once. We augment the original dataset to include these counterfactual songs, $T = T_{OG} \bigcup T_{CF}$. Then, we use five methods to learn the item level representations: one baseline recommender, PinSage, and four bias mitigation methods, ZeroSum \cite{rhee_countering_2022}, MACR \cite{wei_model_2021}, REDRESS, and BOOST. We apply 2-dimensional PCA to each embedding set and analyze the Euclidean distance between the centroids of original track embeddings, $\bar{T}_{OG}$, and counterfactual track embeddings, $\bar{T}_{CF}$. As shown in Figure \ref{fig:cf_emb}, we find that all fairness interventions decrease the distance between the two centroids. Furthermore, as the granularity of fairness increases, the distance between the centroids of learned representations decreases. For example, PinSage, which has no mitigation of popularity bias, has the largest distance of $0.172$. ZeroSum \cite{rhee_countering_2022}, which considers group fairness, decreases the distance to $0.143$, MACR \cite{wei_model_2021}, which uses counterfactual estimation, shrinks to $0.055$. However, the lowest distance achieved is with our proposed approach, i.e., REDRESS and BOOST, with $0.010$. Furthermore, as shown in the orientation of the two song clouds, we can see that, unlike both PinSage and ZeroSum, REDRESS is able to achieve the correct orientation between the two spaces. 
\subsection{RQ2: Do the effects of individual fairness propagate to the producer (artist) level?}
% \rebecca{still experimenting with aggregate stats. if I don't find the right values, I'll move this from Results to Discussion}
\begin{table}[h]
\vspace{-1.5em}
    \centering
    \footnotesize
    \begin{tabular}{|c|c|}
    \hline
         Method  &
         Average Popularity of Top 100 Closest Artists \\ 
    \hline 
    \hline
    REDRESS & 1.091 \\
    BOOST & 1.091 \\ 
    PinSage & 1.115 \\ 
    MACR & 1.172 \\ 
    ZeroSum & 1.192\\ 
    \hline 
    \end{tabular}
    \caption{\textbf{Average Popularity of The top 100 artists (based on embedding)}: We generate artist level representations by averaging all their associated songs. Then, for each embedding method, we use cosine similarity to find the $100$ closest artists and calculate their average popularity. We see that REDRESS and BOOST show the lowest average artist popularity meaning they are robust to popularity bias because these methods select more niche artists when choosing the nearest neighbors for artists in the highest popularity group.}
    \label{table:beatles}
\end{table}
%\vspace{-7mm}
\noindent Building on the analysis in the previous research question, we evaluate whether item level individual fairness can also affect artist (producer) level similarities. To address this question, first, we calculate artist level embeddings by averaging the song embeddings associated with each artist among various embedding sets. For each artist, popularity is calculated using the same procedure outlined in Section \ref{sec:pop_def}. Using these artist-level embeddings, we apply cosine similarity to find the $100$ most similar artists in the embedding space of each algorithm and calculate the average popularity of the artists selected for each grouping. Table \ref{table:beatles} presents the average popularity of the nearest neighbors selected for the artists in the top popularity bin. Similar to the previous question, we observe that both REDRESS and BOOST select more nearest artists from lower popularity bins than other methods.
\subsection{RQ3: How does our individual fairness approach compare to existing methods for mitigating popularity bias?}
\begin{table} [h]
\centering
\footnotesize
\resizebox{\linewidth}{!}{
\begin{tabular}{|ll|cc|cc|cccc|}
\hline && \multicolumn{2}{|c|}{\textbf{Classic}}  
& \multicolumn{2}{|c|}{\textbf{Music}} 
&  \multicolumn{4}{|c|}{\textbf{Fairness}} \\ 
\hline 
\textbf{Data} & \textbf{Model} & 
      Recall@100 & 
      NDCG@100 & 
       Artist Recall@100 & 
      Flow &
      Diversity &
      \%LT &
      LT Cvg &
      Artist Cvg \\
\hline 
\hline 
\multirow{9}{4em}{\textbf{MPD}}&\textbf{Features}  & 
    0.041 & 
    0.073 & 
    0.073 &
    0.900 & 
    0.841 & 
    \textbf{0.588} & 
    0.022 &  
    0.073 \\ 
&\textbf{MostPop}  & 
    0.044 & 
    0.048 & 
    0.141 &
    0.908 & 
    0.680 & 
    0.0 & 
    0.0 &  
    0.001 \\ \cline{2-10}

&\textbf{LightGCN}&
      \textbf{0.106 $\pm$ 0.004} & 
      0.119 $\pm$ 0.004&
       \textbf{0.272 $\pm$ 0.011} & 
      0.905 $\pm$ 0.000& 
      0.672 $\pm$ 0.025&
      0.002 $\pm$ 0.000& 
      0.000 $\pm$ 0.000& 
      0.025 $\pm$ 0.001\\ 
& \textbf{PinSage} & 
    0.068 $\pm$ 0.002 & 
     \textbf{0.144 $\pm$ 0.003} & 
    0.139 $\pm$ 0.003 &
    0.931 $\pm$ 0.001 & 
    0.707 $\pm$ 0.003 & 
    0.476 $\pm$ 0.002 &  
    0.032 $\pm$ 0.000 &  
    0.105 $\pm$ 0.000 \\ \cline{2-10}
% \hline 
 % &\textbf{ZeroSum}   &  %G_0.8
 %    0.000 $\pm$ 0.000& 
 %    0.000 $\pm$ 0.000& 
 %    0.014 $\pm$ 0.001&
 %    0.873 $\pm$ 0.000& 
 %    0.993 $\pm$ 0.010& 
 %    0.836 $\pm$ 0.005& 
 %    0.048 $\pm$ 0.001&  
 %    0.134 $\pm$ 0.002 \\
    
&\textbf{ZeroSum}   &  %G_0.1
    0.044 $\pm$ 0.002& 
    0.043 $\pm$ 0.002& 
    0.220 $\pm$ 0.008 &
    0.904 $\pm$ 0.001& 
    0.765 $\pm$ 0.013& 
    0.000 $\pm$ 0.003& 
    0.000 $\pm$ 0.000&  
    0.048 $\pm$ 0.002 \\
 

&\textbf{xQuAD}  & %G_0.1
    0.064 $\pm$ 0.005 & 
    0.104 $\pm$ 0.006 & 
    0.135 $\pm$ 0.013&
    0.927 $\pm$ 0.004& 
    0.703 $\pm$ 0.059& 
    0.226 $\pm$ 0.001& 
    0.017 $\pm$ 0.000&  
    0.098 $\pm$ 0.004 \\ 

&\textbf{MACR}  & %C=5
    0.028 $\pm$ 0.014& 
    0.030 $\pm$ 0.015& 
    0.149 $\pm$ 0.022&
    0.902 $\pm$ 0.002& 
    0.831 $\pm$ 0.034& 
    0.019 $\pm$ 0.006& 
    0.000 $\pm$ 0.001&  
    0.011 $\pm$ 0.003 \\ \cline{2-10}
& \textbf{ReDress}  & %(G=0.5)
    0.045 $\pm$ 0.002 & 
    0.100 $\pm$ 0.003 & 
    0.162 $\pm$ 0.004 &
    0.969 $\pm$ 0.032& 
    0.829 $\pm$ 0.001& 
    0.504 $\pm$ 0.003& 
    0.036 $\pm$ 0.004 &  
    0.117 $\pm$ 0.000 \\ 
% \hline
&  \textbf{BOOST} & 
    0.020 $\pm$ 0.004 & %(G=0.5)
    0.047 $\pm$ 0.003& 
    0.137 $\pm$ 0.002 &
    \textbf{0.979 $\pm$ 0.000} & 
    \textbf{0.899 $\pm$ 0.002}& 
    \textbf{0.522 $\pm$ 0.001}& 
    \textbf{0.037 $\pm$0.003}&  
    \textbf{0.125 $\pm$0.000} \\
\hline 
&  \textit{p values} & 
    4.408083e-16	 & 
    1.768725e-19& 
    0.727897	 &
    3.751961e-61 & 
    1.168816e-29 & 
    0.000596& 
    -&  
    -  \\
% &  \textbf{BOOST} & 
%     0.010 $\pm$ 0.004 & %(G=0.8)
%     0.027 $\pm$ 0.003& 
%     0.108 $\pm$ 0.002 &
%     0.983 $\pm$ 0.000 & 
%     0.915 $\pm$ 0.002& 
%     0.569 $\pm$ 0.001& 
%     0.041 $\pm$0.003&  
%     0.132 $\pm$0.000 \\
\hline
\hline 

\multirow{9}{4em}{\textbf{LFM}}&\textbf{Features}  & 
    0.033 & 
    0.037 & 
    0.041 &
    0.996 & 
    0.919 & 
    0.486 & 
    0.005 &  
    0.034 \\
 &\textbf{MostPop}  & 
    0.015 & 
    0.011 & 
    0.046 &
    0.926 & 
    0.600 & 
    0.000 & 
    0.000 &  
    0.001 \\ \cline{2-10}
&\textbf{LightGCN} &
      0.026 $\pm$ 0.001	 & 
      0.023	 $\pm$ 0.001	&
      0.068 $\pm$ 0.001	& 
      0.998$\pm$ 0.000 & 
      0.505 $\pm$ 0.012&
      0.000 $\pm$ 0.000& 
      0.000 $\pm$ 0.000& 
      0.003 $\pm$ 0.001	\\ 
& \textbf{PinSage} & 
    \textbf{0.064 $\pm$ 0.001} & 
    \textbf{0.095 $\pm$ 0.002} & 
    \textbf{0.077  $\pm$ 0.002} &
    0.969 $\pm$ 0.000 & 
    0.775 $\pm$ 0.003 & 
    0.437 $\pm$ 0.001 &  
    0.008  $\pm$ 0.000 &  
    0.053  $\pm$ 0.001 \\ \cline{2-10}
&\textbf{ZeroSum}  & %G = 0.5
    0.001 $\pm$ 0.003& 
    0.001 $\pm$ 0.001& 
    0.045 $\pm$ 0.004&
    0.996 $\pm$ 0.008& 
    0.866 $\pm$ 0.000& 
    0.007 $\pm$ 0.000& 
    0.000 $\pm$ 0.000&  
    0.032 $\pm$ 0.001 \\
    
& \textbf{xQuAD} & %g_0.1
    0.055 $\pm$ 0.001 & 
    0.064 $\pm$ 0.001 & 
    0.068 $\pm$ 0.002 &
    0.998 $\pm$ 0.000 & 
    0.801 $\pm$ 0.008 & 
    0.212 $\pm$ 0.000 & 
    0.004 $\pm$ 0.000 &  
    0.053 $\pm$ 0.001 \\

&\textbf{MACR}  & %G = 5
    0.014 $\pm$ 0.001& 
    0.014 $\pm$ 0.001& 
    0.049 $\pm$ 0.007&
    0.996 $\pm$ 0.003& 
    0.777 $\pm$ 0.050& 
    0.002 $\pm$ 0.004& 
    0.000 $\pm$ 0.000&  
    0.001 $\pm$ 0.000 \\ \cline{2-10}
    
&\textbf{ReDress} & %(G = 0.2)
    0.038 $\pm$ 0.002 & 
    0.053 $\pm$ 0.004 & 
    0.057 $\pm$ 0.001 &
    0.998 $\pm$ 0.002& 
    0.862 $\pm$ 0.004& 
    0.451 $\pm$ 0.000& 
    0.008 $\pm$ 0.002&  
    0.056 $\pm$ 0.000 \\

% %(G = 0.8)
%     0.009 $\pm$ 0.002 & 
%     0.011 $\pm$ 0.004 & 
%     0.029 $\pm$ 0.001 &
%     0.999 $\pm$ 0.000& 
%     0.923 $\pm$ 0.004& 
%     0.491 $\pm$ 0.000& 
%     0.010 $\pm$ 0.001&  
%     0.066 $\pm$ 0.000 \\

 &\textbf{Boost}  & 
    0.005 $\pm$ 0.001&  %(G=0.6)
    0.007 $\pm$ 0.001& 
    0.029 $\pm$ 0.002&
    \textbf{0.999 $\pm$ 0.000} & 
    \textbf{0.941 $\pm$ 0.003} & 
    \textbf{0.498 $\pm$ 0.006} & 
    \textbf{0.010 $\pm$ 0.000} &  
    \textbf{0.068 $\pm$ 0.001} \\ 
\hline 
&  \textit{p values} & 
    5.696989e-08	 & 
    1.179627e-15& 
    1.914129e-07&
    0.001408 & 
    1.112495e-34&  
    2.477700e-11& 
    -&  
    - \\
\hline 
\end{tabular}
}
\caption{Comparison Between All Methods}
\label{table:baseline_comp}
\vspace{-6mm}
\end{table}
Having illustrated the benefits of domain aware individual fairness, we compare our method with five baselines. Our motivation for selecting these particular baselines is to showcase the improvements that our method can have on a broad scale. The \textbf{Features} baseline showcases the improvements that PinSage, REDRESS, and BOOST contribute by integrating structural information into the recommendations. \textbf{ZeroSum} \cite{rhee_countering_2022} and \textbf{MACR} \cite{wei_model_2021} show comparisons with two in-processing methods that use group and counterfactual fairness to mitigate popularity bias. Finally, \textbf{Smooth xQuAD} shows the improvements that a re-ranking approach can contribute to the mitigation of popularity bias. 


In Table \ref{table:baseline_comp} we show a side by side comparison of the various recommendation and fairness methods. To test the significance of our proposed BOOST method, we apply the Wilcoxon signed-rank test \cite{rey_wilcoxon-signed-rank_2011} to these playlists, and metric pairs and include the $p$ values. In order to select the best performance among a vector of performance and fairness metrics, we calculate the values of $<\textit{Recall, NDCG, Artist Recall, \%LT, and LT Cvg}>$, apply a min-max scaling, and average the metrics. We select the model based on the maximum average performance and then report the associated results within the test set. For each fairness baseline, there is a hyperparameter which tunes the balance between fairness intervention and performance. In Table \ref{table:baseline_comp}, we select only the best value of $\gamma$. However, we also present the Pareto plots exploring the entire range of the values in Figure \ref{fig:pareto_plots}. 

\begin{figure} [h]
\centering
\includegraphics[width=.4\linewidth]{Viz/PARETO/LFM_Pareto_clean.png}
\includegraphics[width=.4\linewidth]{Viz/PARETO/MPD_Pareto.png}
\includegraphics[scale=0.3]{Viz/legend.png}
\caption{\textbf{Plots showing the effects of fairness intervention method on performance/fairness metrics}: we show the effects of tuning a hyperparameter to balance fairness and performance in each of our fairness methods, we explore the entire range of the values and report the trade-off that increasing this fairness intervention can have. Note, that REDRESS has the best robustness with respect to balancing recall and \%LT. }
\label{fig:pareto_plots}
\end{figure}



% As we see Table \ref{table:fairness_comp}, the definition of popularity plays a significant role in the model selection method \textit{especially} in the case where user preferences encoded in the training data skew towards popular items. Defining a wider window for unpopular items can synthetically inflate the performance of $\%LT$ and $LT Cvg$. For example, in the case of the LFM dataset, in which user preferences are skewed towards songs of mid level popularity, we can see that using a long tail model (unscaled, 20/80 split) can indicate that xQuAD has the best $\%LT$ performance even when this is not the case in our, more granular, formulation. This is even better visualized by Figure \ref{fig:group_plots} where we can see that methods like xQuAD and ZeroSum are selecting a majority of their items from bins 1,2 or 3. Had we used the classical long tail methodology, these differences would not be visible, masking the important differences among the baselines. 

% \begin{figure}[H]
% \centering
% \includegraphics[width=.3\textwidth]{Viz/LFM_grouped.png}
% \includegraphics[width=.3\textwidth]{Viz/MPD_grouped.png}
% \caption{Group By Group Analysis of Recommendations}
% \label{fig:group_plots}
% \end{figure}

% It is interesting to note that, even within the sphere of different formulations, both REDRESS and BOOST show relatively high, if not always top performance. For example, in the MPD dataset, although the bare features achieve the best fairness performance, BOOST is a close second. 



==> Sections/Old_Versions/06discussion.tex <==
\section{Discussion} \label{sec:discussion}
In this section we unpack the key findings from the results presented above. First, we motivate our selection of PinSage and highlight the effects of model selection on the mitigation of popularity bias. Second, we analyze the connection between our method's musical domain awareness and the achieved fairness performance. Then, we highlight the strengths of our popularity definition by showing a detailed breakdown of each method's performance with respect to our previously defined popularity bins. Finally, we detail the potential limitations of our methodology, highlighting a few areas for future work. 

\noindent \textbf{Model Agnostic Approaches to Fairness}: First, we investigate whether fairness should be considered from a model agnostic standpoint. As we show in Table \ref{table:baseline_comp}, we can see that simply the decision between LightGCN \cite{he_lightgcn_2020} and PinSage \cite{ying_graph_2018} has important consequences on the baseline fairness achieved in the recommendation results. With respect to the classic performance metrics, $Recall$ and $NDCG$, we see that the baseline recommenders, PinSage and LightGCN have the best performance among all the methods. We note that for the case of MPD, LightGCN outperforms PinSage on both song and artist based $Recall$ while on LFM PinSage outperforms LightGCN for both of the metrics. This can be attributed to the inductive nature of the cold start setting. That is, LightGCN is not intended for a setting in which a test user (or playlist) lacks extensive interaction data. Thus, in the LFM setting,  PinSage demonstrates a more robust performance. Furthermore, as shown on both datasets, PinSage (without any mitigation) has a significantly higher percentage of long tail items and artists. We hypothesize that this can be attributed to differences in the PinSage/LightGCN architectures. As explained in Section \ref{sec:GNN_in_rec}, while LightGCN learns user and item embeddings simultaneously,  PinSage only learns item (song) embeddings. While it is clear that learning embeddings simultaneously allows for improved performance on classic recommendation metrics, it can also create biases against long tail information and deteriorate the performance of an algorithm in a cold start setting. Thus, it is important to consider not just the approach to mitigating bias but also the underlying model that the approach is compatible with. 

\begin{figure}[h]
\vspace{-4mm}
\centering
\includegraphics[scale=.2]{Viz/CIRCLE/MPD_circle.png}
\includegraphics[scale=.2]{Viz/CIRCLE/LFM_circle.png}
\caption{Performance Breakdown by Fairness Model}
\label{fig:circle_plots}
\vspace{-2mm}
\end{figure}

\noindent \textbf{Importance of Music Features}: There is an influential body of work showing that content-based methods are less prone to popularity bias than consumption-based methods \cite{celma_from_2008, deldjoo_ContentdrivenMR_2021}. It is from this perspective that we choose to ground our method in music features. As we show in Figure \ref{fig:pareto_plots}, on both datasets, REDRESS outperforms the other fairness methods and the integration of our BOOST methodology further improves this performance. In Figure \ref{fig:circle_plots} we observe that REDRESS and BOOST have a more robust performance on the fairness metrics compared to the baselines. Furthermore, our method is able to have high values in both coverage and percentage of long tail items meaning that REDRESS/BOOST is not just prioritizing niche items but also choosing a diverse selection from this category. We attribute the relative gains of REDRESS and BOOST to their ability to integrate musical features into their fairness mitigation because they are able to select not just niche items, but also musically relevant ones for recommendation. Finally, our method's ability to interpolate between these two perspectives of content and consumption patterns, shows that REDRESS/BOOST is able to recommend similar ratios of niche items compared to the bare features while having significantly better performance.  \\ 

\noindent \textbf{Dataset Selection}: We notice a significantly steeper drop in the performance/fairness tradeoff on the LFM dataset. This can be attributed to two distinctions between the  datasets. First, as mentioned in earlier sections, the implicit nature of LFM's interaction feedback means that the dataset is significantly noisier. Second, by looking at the user preferences among various popularity groups within the training set, we can see that in LFM there is a noticeable skew towards mid-tier popular items (see Figure \ref{fig:dset_breakdown}). Thus, any increase in niche recommendations will show a more significant drop in classic performance metrics. This highlights the importance of evaluating a method on both implicit and explicit interactions to simulate the utility and fairness performance as it will be enacted in each feedback setting. 
\begin{figure}[h]
\centering
\includegraphics[width=.45\textwidth]{Viz/GROUP_BY_GROUP/LFM_recs.png}
\includegraphics[width=.45\textwidth]{Viz/GROUP_BY_GROUP/MPD_recs.png}
\caption{\textbf{Group By Group Analysis of Recommendations}: we look at a breakdown of the recommendations for each dataset. We define visibility as the number of times an item from this group appears in the recommendations normalized by the total number of items in the recommendation lists. Bins are defined using the metheodology of Section \ref{sec:pop_def} where bin $0$ has the lowest popularity.}
\label{fig:group_plots}
\vspace{-6mm}
\end{figure}

\noindent\textbf{Popularity Definition}: As we can see in Figure \ref{fig:group_plots} the definition of popularity plays a significant role in the model selection method \textit{especially} in the case where user preferences encoded in the training data skew towards popular items. Defining a wider window for defining unpopular items can synthetically inflate the performance of $\%LT$ and $LT Cvg$. For example, we can see that methods like xQuAD and ZeroSum are selecting a majority of their items from bins 1,2 or 3. Using a classical long tail methodology, these differences would not be as visible, masking distinctions among the baselines' fairness. Furthermore, this visualization provides insight into the different stages of popularity bias at which various methods perform best. For example, MACR was proposed not explicitly as a method for promoting fairness but rather as a method for improving overall performance. Thus, this method is able to improve visibility for some lower end items, but it mostly focuses on relevance. Meanwhile, xQuAD is intended for increasing diversity so it is able to select from lower bins than ZeroSum or MACR. 


\noindent\textbf{Limitations of Our Work  \& Future Work}: Due to the nature of publicly available data, both of these datasets skew heavily towards Western, anglophone content and are not representative of the wide array of music that is available for consumption. Furthermore, it is important to remember that recommender systems are responsible for serving the tastes of listeners, not policing them, and we do not deny the validity of mainstream listening practices. Given our focus on the mitigation of bias, we cannot say how well our method serves the tastes of different listener profiles and whether our mitigation technique might affect those with majoritarian tastes. We leave this deeper user preference analysis for future work. Finally, we note that given the fairness focus of this work, we do not explore methods for improving the performance of PinSage. For example, our method for generating recommendations can certainly be more complex. We leave this, and other architecture improvements, for future work. 

==> Sections/Old_Versions/06discussion_CUT.tex <==
% \section{Discussion} \label{sec:discussion}
% In this section we unpack the key findings from the results presented above. First, we motivate our selection of PinSage and highlight the effects of model selection on the mitigation of popularity bias. Second, we analyze the connection between our method's musical domain awareness and the achieved fairness performance. Then, we highlight the strengths of our popularity definition by showing a detailed breakdown of each method's performance with respect to our previously defined popularity bins. Finally, we detail the potential limitations of our methodology, highlighting a few areas for future work. 

% \noindent \textbf{Model Agnostic Approaches to Fairness}: First, we investigate whether fairness should be considered from a model agnostic standpoint. As we show in Table \ref{table:baseline_comp}, we can see that simply the decision between LightGCN \cite{he_lightgcn_2020} and PinSage \cite{ying_graph_2018} has important consequences on the baseline fairness achieved in the recommendation results. With respect to the classic performance metrics, $Recall$ and $NDCG$, we see that the baseline recommenders, PinSage and LightGCN have the best performance among all the methods. We note that for the case of MPD, LightGCN outperforms PinSage on both song and artist based $Recall$ while on LFM PinSage outperforms LightGCN for both of the metrics. This can be attributed to the inductive nature of the cold start setting. That is, LightGCN is not intended for a setting in which a test user (or playlist) lacks extensive interaction data. Thus, in the LFM setting,  PinSage demonstrates a more robust performance. Furthermore, as shown on both datasets, PinSage (without any mitigation) has a significantly higher percentage of long tail items and artists. We hypothesize that this can be attributed to differences in the PinSage/LightGCN architectures. As explained in Section \ref{sec:GNN_in_rec}, while LightGCN learns user and item embeddings simultaneously,  PinSage only learns item (song) embeddings. While it is clear that learning embeddings simultaneously allows for improved performance on classic recommendation metrics, it can also create biases against long tail information and deteriorate the performance of an algorithm in a cold start setting. Thus, it is important to consider not just the approach to mitigating bias but also the underlying model that the approach is compatible with. 

% % \begin{figure}[h]
% % \vspace{-4mm}
% % \centering
% % \includegraphics[width=\columnwidth]{Viz/CIRCLE/MPD_circle.png}
% % \includegraphics[width=\columnwidth]{Viz/CIRCLE/LFM_circle.png}
% % \caption{Performance Breakdown by Fairness Model}
% % \label{fig:table}
% % \vspace{-2mm}
% % \end{figure}

% \noindent \textbf{Importance of Music Features}: There is an influential body of work showing that content-based methods are less prone to popularity bias than consumption-based methods \cite{celma_from_2008, deldjoo_ContentdrivenMR_2021}. It is from this perspective that we choose to ground our method in music features. As we show in Figure \ref{fig:pareto_plots}, on both datasets, REDRESS outperforms the other fairness methods and the integration of our BOOST methodology further improves this performance. We observe that REDRESS and BOOST have a more robust performance on the fairness metrics compared to the baselines. Furthermore, our method is able to have high values in both coverage and percentage of long tail items meaning that REDRESS/BOOST is not just prioritizing niche items but also choosing a diverse selection from this category. We attribute the relative gains of REDRESS and BOOST to their ability to integrate musical features into their fairness mitigation because they are able to select not just niche items, but also musically relevant ones for recommendation. Finally, our method's ability to interpolate between these two perspectives of content and consumption patterns, shows that REDRESS/BOOST is able to recommend similar ratios of niche items compared to the bare features while having significantly better performance.  \\ 

% \noindent \textbf{Dataset Selection}: We notice a significantly steeper drop in the performance/fairness tradeoff on the LFM dataset. This can be attributed to two distinctions between the  datasets. First, as mentioned in earlier sections, the implicit nature of LFM's interaction feedback means that the dataset is significantly noisier. Second, by looking at the user preferences among various popularity groups within the training set, we can see that in LFM there is a noticeable skew towards mid-tier popular items (see Figure \ref{fig:dset_breakdown}). Thus, any increase in niche recommendations will show a more significant drop in classic performance metrics. This highlights the importance of evaluating a method on both implicit and explicit interactions to simulate the utility and fairness performance as it will be enacted in each feedback setting. 
% \begin{figure}[h]
% \centering
% \includegraphics[width=.45\columnwidth.]{Viz/GROUP_BY_GROUP/LFM_recs.png}
% \includegraphics[width=.45\columnwidth.]{Viz/GROUP_BY_GROUP/MPD_recs.png}
% \caption{\textbf{Group By Group Analysis of Recommendations}: we look at a breakdown of the recommendations for each dataset. We define visibility as the number of times an item from this group appears in the recommendations normalized by the total number of items in the recommendation lists. Bins are defined using the metheodology of Section \ref{sec:pop_def} where bin $0$ has the lowest popularity.}
% \label{fig:group_plots}
% \vspace{-6mm}
% \end{figure}

% \noindent\textbf{Popularity Definition}: As we can see in Figure \ref{fig:group_plots} the definition of popularity plays a significant role in the model selection method \textit{especially} in the case where user preferences encoded in the training data skew towards popular items. Defining a wider window for defining unpopular items can synthetically inflate the performance of $\%LT$ and $LT Cvg$. For example, we can see that methods like xQuAD and ZeroSum are selecting a majority of their items from bins 1,2 or 3. Using a classical long tail methodology, these differences would not be as visible, masking distinctions among the baselines' fairness. Furthermore, this visualization provides insight into the different stages of popularity bias at which various methods perform best. For example, MACR was proposed not explicitly as a method for promoting fairness but rather as a method for improving overall performance. Thus, this method is able to improve visibility for some lower end items, but it mostly focuses on relevance. Meanwhile, xQuAD is intended for increasing diversity so it is able to select from lower bins than ZeroSum or MACR. 


\noindent\textbf{Limitations of Our Work  \& Future Work}: Due to the nature of publicly available data, both of these datasets skew heavily towards Western, anglophone content and are not representative of the wide array of music that is available for consumption. Furthermore, it is important to remember that recommender systems are responsible for serving the tastes of listeners, not policing them, and we do not deny the validity of mainstream listening practices. Given our focus on the mitigation of bias, we cannot say how well our method serves the tastes of different listener profiles and whether our mitigation technique might affect those with majoritarian tastes. We leave this deeper user preference analysis for future work. Finally, we note that given the fairness focus of this work, we do not explore methods for improving the performance of PinSage. For example, our method for generating recommendations can certainly be more complex. We leave this, and other architecture improvements, for future work. 
